Relation between charging times and storage properties of nanoporous supercapacitors

Investigating the correlations between dynamic and static storage properties of nanoporous electrodes is beneficial for further progress of supercapacitors-based technologies. While the dependence of the capacitance on the pores' sizes is well described by classical Density Functional Theory (c-DFT), the lack of dynamic c-DFT extension capable for correct estimation of the charging time has been noted in the literature. Here, we develop a dynamic model of the electrolyte inside nanopores based on c-DFT and realistically describing both the time-dependent charging process and maximum static capacitance. Our calculations show that the charging starts with a square-root dependency of the total charge on time and then follows two subsequent exponential trends with significantly different time scales that agree with published simulations. We demonstrate that the full charging time corresponds to the timescale of either the first or the second exponential trend depending on the pores' size. Also, we find analytical expressions to fit the timescales for a wide range of parameters. Derived correlations provide the relation of charging time to pores' size, applied voltage, and final ions' densities inside the pore, making these expressions useful to design supercapacitors with an optimal combination of power and energy characteristics.

==> sections/appendices/analytics.tex <==
\section{Analytical derivation}
\subsection{Pressure}
The Gibbs-Duhem equation shows how the component chemical potentials relate to the pressure:
\begin{equation}
\label{eq:Gibbs-Duhem}
VdP=N_1d\mu_1+N_2d\mu_2
\end{equation}
After substitution of Gibbs-Duhem relation in terms of the average densities $\overline{\rho}_i=N_i/V$ the dynamic equation can be rewritten as follows
\begin{equation}
\partial_t (\overline{\rho}_1+\overline{\rho}_2)=D\beta\partial_x (\overline{\rho_1}\partial_x \mu_1+\overline{\rho_2}\partial_x \mu_2)=D\beta \partial_x^2 P(\overline{\rho}_1,\overline{\rho}_2) \nonumber
\end{equation}
The Helmholtz free energy can be rewritten as follows: 
\begin{align}
\label{eq:}
F=F_\text{id}+F_\text{hs}+F_\text{el}+k T\sum_i\int dr\rho_i(r)U_{C,i}(r)+ \nonumber 
\\
\sum_i A\int dz \rho_i(z)\left[U_{w,i}(z)+U_{w,i}(H-z)+Z_i e\psi(z,H)\right]
\end{align}
We denote the terms which depend on the $H$ explicitly as $U_{ext}(z,H)$, then
\begin{equation}
\rho_i(z)=\frac{\delta F}{\delta U_{ext}(z,H)}=\frac{\delta \Omega}{\delta U_{ext}(z,H)}
\end{equation}
The confined pressure in the open system is derived from the following volume derivative:
\begin{widetext}
\begin{align}
    \psi(z)=U_0+\frac{4\pi l_\text{B} z}{H}\int_0^H (H-z')\sum_{k=1}^n Z_k \rho_k(z')dz'
-4\pi l_\text{B}\int_0^z(z-z')\sum_{k=1}^n Z_k \rho_k(z')dz' 
%= \nonumber \\
%=U_0+2\pi l_B z H\int_0^1d\xi q(\xi)-4\pi l_\text{B}\int_0^z(z-z')\sum_{k=1}^n Z_k \rho_k(z')dz' \nonumber 
\\
\frac{d\psi(z,H)}{d H}=-\frac{4\pi l_B z}{H^2} \int_0^H dz' (H/2+H/2-z')q(z')+0+\frac{4\pi l_B z}{H}\int_0^Hdz'q(z')=-\frac{2\pi l_B z}{H}Q
\end{align}
\begin{align*}
P=-\frac{d\Omega}{d V}=-\sum_i\int_{0}^H dz \rho_i(z)\frac{d U_{ext}(z,H)}{d H}
=-\sum_i\int_{0}^H dz \rho_i(z)\frac{d}{d H} \left[ \theta(-z+d/2)+\theta(z-H+d/2)+Z_i e \psi(z,H)\right]= \nonumber\\
=
%\rho(d/2)-Z_i 4\pi l_B  e \int_{0}^Hz\rho_i(z)dz\left[-\frac{1}{H^2}\int_0^Hdz'(H/2+H/2-z')q(z')+\frac{1}{H}\int_{0}^Hdz'q(z')\right]=\rho(d/2)-\frac{2\pi l_B (-Q)}{H}\int_0^H dz z q(z)= \nonumber \\
\rho(d/2)+\frac{2\pi l_B Q}{H}\int_0^Hdz z\sum_i Z_i\rho_i(z)
=\rho(d/2)-\frac{Q}{2H}\int_0^H dz z \psi''(z) \nonumber \\
=\rho(d/2)-\frac{Q}{2H}\left[ H \psi'(H)-\int_0^Hdz\psi'(z)\right]=\rho(d/2)+\frac{Q}{2}\psi'(0)=\rho(d/2)-2\pi l_B \frac{Q^2}{2}
\end{align*}
\end{widetext}
The system of charge hard spheres exhibits the following pressure:
\begin{equation}
\label{eq:pressure}
\beta P= \rho_1(d/2)+\rho_2(d/2)-\frac{Q^2}{2\epsilon_0\epsilon k T}=\rho(d/2)-2\pi\frac{Q^{*2}\lambda_B}{d^4}
\end{equation}
\begin{equation}
\rho_i(d/2)=\rho_i^{(0)}\exp\left[-Z_i U_0^*+Z_i \pi\lambda_B Q^*-\beta \Delta\mu_i^{\text{exc}}|_{z=d/2}\right] \nonumber
\end{equation}

\subsection{Linearization near the final state}
In order to describe charging dynamics at the later stage, one can linearize the transport equations \eqref{eq:transport_average} near the final steady-state solution $\bar{\rho}_i (x, t) = \bar{\rho}^{f}_{i} + \bar{\rho}'_{i}$, $\bar{\rho}^{f}_{i}~=~const$ to get the system $\partial_t \bar{\rho}'_i - D_{ij} \partial_{xx} \bar{\rho}'_j = 0$ for the small corrections of densities $\rho'_i$ to the final steady-state solution. Here the matrix $D$ is given by
\begin{equation*}
D = \left.
\begin{pmatrix}
\bar{\rho}_1 \dfrac{\partial \mu_1}{\partial \bar{\rho}_1} & \bar{\rho}_1 \dfrac{\partial \mu_1}{\partial \bar{\rho}_2} \\
\bar{\rho}_2 \dfrac{\partial \mu_2}{\partial \bar{\rho}_1} & \bar{\rho}_2 \dfrac{\partial \mu_2}{\partial \bar{\rho}_2}
\end{pmatrix} \right|_{\bar{\rho}_i = \bar{\rho}^f_i}.
\end{equation*}

Using the Gibbs-Duhem relation \eqref{eq:Gibbs-Duhem} one can prove that the cross-derivatives of the chemical potentials with respect to average densities are equal
\begin{equation*}
\dfrac{\partial \mu_1}{\partial \bar{\rho}_2} = \dfrac{\partial \mu_2}{\partial \bar{\rho}_1}.
\end{equation*}
Utilizing the latter identity one can also show that the discriminant of the characteristic polynomial of the matrix $D$ is positive, the matrix has distinct real eigenvalues $\lambda_{1,2}$ and complete system of eigenvectors $\Omega$ and, thus, is diagonalizable $D = \Omega^{-1} \Lambda \Omega$, $\Lambda = \mathrm{diag} (\lambda_1, \lambda_2)$. Multiplication of the linearized equations by $\Omega$ gives the system of {\it decoupled} linear diffusion equations for linear combinations of corrections $\bar{\rho}'_i$. Since the boundary conditions for the corrections are essentially the same as for $\bar{\rho}_i$ (given value $\bar{\rho}'_i = 0$ at $x = 0$ and zero flux $\partial_x \bar{\rho}'_i = 0$ at $x = L$), the same is valid for those linear combinations. Accordingly, the TLM solution discussed above can be applied for both equations independently and it will result in two different timescales $\tau_{1,2}$ defined by the corresponding eigenvalues.

The eigenvalues $\lambda_{1,2}$ are given by
\begin{equation*}
\lambda_{1,2} = \dfrac{1}{2} \left(\mathrm{tr} D \pm \sqrt{(\mathrm{tr} D)^2 - 4 \mathrm{det} D}\right).
\end{equation*}

The ratio of the eigenvalues $\lambda$ is a function of the ratio $\mathrm{det} D / (\mathrm{tr} D)^2$ only. It can be shown that $\lambda \ll 1 \Leftrightarrow \mathrm{det} D / (\mathrm{tr} D)^2 \ll 1$. Furthermore, if the ideal gas contribution in \eqref{eq:pressure} is small compared to charge term, one can show that 
\begin{equation}
\label{eq:det_tr2}
\frac{\mathrm{det} D}{(\mathrm{tr} D)^2} = c (1 - c) \left(\frac{\mu}{(c + (1 - c) \mu)^2} - 1\right).
\end{equation}
Here 
\begin{equation*}
c = \frac{\bar{\rho}_1}{\bar{\rho}_1 + \bar{\rho}_2}, \quad \mu = \frac{\partial \mu_2}{\partial \bar{\rho}_2} / \frac{\partial \mu_1}{\partial \bar{\rho}_1}.
\end{equation*}
The expression \eqref{eq:det_tr2} has four zero-curves at $c-\mu$ plane: $c = 0$,  $c = 1$, $\mu = 1$ and $\mu = \mu^*(c)$. 

Accordingly, for large charges ($P \sim Q^2$) and low fractions of co-ions ($c \approx 1$) the ratio of the eigenvalues is small $\lambda \ll 1$ independent of chemical potential derivatives. It also may happen for certain very special conditions $\mu \approx 1$ and $\mu \approx \mu^*(c)$ (again, as long as $P \sim Q^2$).

\subsection{Calculation of the chemical potential derivatives}
Equations for the equilibrium distributions of densities in transverse direction may be written as
$\mu_i = \log \rho_i + G_i$ or equivalently as $\rho_i = \exp (\mu_i) F_i$, where $F_i = \exp (-G_i)$. Integrating over the pore width one can eliminate the chemical potentials and get the equations for density distributions in terms of average densities only
\begin{equation*}
\rho_i = \bar{\rho}_i \dfrac{F_i}{\bar{F_i}}, \quad \bar{F}_i = \int^1_0 dz \; F = \int^1_0 dz \; \exp(-G_i).
\end{equation*}
Differentiation of both sides of the equation with respect to the average densities and algebraic transformations give
\begin{gather*}
\bar{\rho}_i \dfrac{\partial \mu_i}{\partial \bar{\rho}_i} = 1 - \bar{\rho}_i \dfrac{\partial}{\partial \bar{\rho}_i} \log \bar{F}_i, \\
\bar{\rho}_i \dfrac{\partial \mu_i}{\partial \bar{\rho}_j} = - \bar{\rho}_i \dfrac{\partial}{\partial \bar{\rho}_j} \log \bar{F}_i, \quad j \neq i
\end{gather*}
\color{red} The question is can we somehow (saddle-point method?) estimate $\log \bar{F}_i$? Or show that
\begin{equation*}
\dfrac{\partial \mu_i}{\partial \bar{\rho}_i} \gg \dfrac{\partial \mu_i}{\partial \bar{\rho}_j}, \quad j \neq i?
\end{equation*}
If the latter is true, eigenvalues are simply diagonal elements.
\color{black}
